MDM-Prime-v2: Binary Encoding and Index Shuffling Enable Scaling of Diffusion Language Models

Masked diffusion models (MDM) exhibit superior generalization when learned using a Partial masking scheme (Prime). This approach converts tokens into sub-tokens and models the diffusion process at the sub-token level. We identify two limitations of the MDM-Prime framework. First, we find that the functional form of the subtokenizer significantly increases the cross-entropy loss in the objective when paired with commonly used Byte-Pair-Encoding (BPE) tokenizers. Second, we lack tools to guide the hyperparameter choice of the token granularity in the subtokenizer. To address these limitations, we analyze the optimal design of the subtokenizer that minimizes MDM-Prime training objective and develop MDM-Prime-v2, a masked diffusion language model which incorporates Binary Encoding and Index Shuffling. Our analysis characterizes how token granularity and sub-token entropy influence the training objective and downstream performance, providing principled criteria for subtokenizer design. When extending the model size to 1.1B parameters, MDM-Prime-v2 demonstrates superior average zero-shot accuracy across eight commonsense reasoning benchmarks, outperforming similar-sized baselines including GPT-Neo, OPT, Pythia, Bloom, SMDM, and TinyLLaMA.

==> figures/text_generation.tex <==
\clearpage
\begin{figure}[t]
    \centering
    \footnotesize
    \setlength{\fboxsep}{-2pt}
    \fcolorbox{gray}{white}{%
        \includegraphics[width=\linewidth]{figures/assets/prefix_2.pdf}
    }
    \caption{(Example 1) Prefix text used for conditional generation, extracted from the QMSum dataset~\cite{zhong2021qmsumnewbenchmarkquerybased}.}
    \label{fig:apx:prefix_2}
\end{figure}

\begin{figure}[t]
    \centering
    \footnotesize
    \setlength{\fboxsep}{-2pt}
    \fcolorbox{gray}{white}{%
        \includegraphics[width=\linewidth]{figures/assets/suffix_2.pdf}
    }
    \caption{(Example 1) Suffix text used for conditional generation, extracted from the QMSum dataset~\cite{zhong2021qmsumnewbenchmarkquerybased}.}
    \label{fig:apx:suffix_2}
\end{figure}

% \clearpage
\begin{figure}[t]
    \centering
    \footnotesize
    \setlength{\fboxsep}{-2pt}
    \fcolorbox{gray}{white}{%
        \includegraphics[width=\linewidth]{figures/assets/reference_2.pdf}
    }
    \caption{(Example 1) The ground-truth reference text extracted from the QMSum dataset~\cite{zhong2021qmsumnewbenchmarkquerybased}.}
    \label{fig:apx:reference_2}
\end{figure}

\begin{figure}[t]
    \centering
    \footnotesize
    \setlength{\fboxsep}{-2pt}
    \fcolorbox{gray}{white}{%
        \includegraphics[width=\linewidth]{figures/assets/prime_response_2.pdf}
    }
    \caption{(Example 1) Conditional sample generated using MDM-Prime-v2 (1.1B).}
    \label{fig:apx:prime_response_2}
\end{figure}



\begin{figure}[t]
    \centering
    \footnotesize
    \setlength{\fboxsep}{-2pt}
    \fcolorbox{gray}{white}{%
        \includegraphics[width=\linewidth]{figures/assets/ar_response_2.pdf}
    }
    \caption{(Example 1) Conditional sample generated using Pythia (1.4B).}
    \label{fig:apx:pythia_response_2}
\end{figure}

\clearpage
\begin{figure}[t]
    \centering
    \footnotesize
    \setlength{\fboxsep}{-2pt}
    \fcolorbox{gray}{white}{%
        \includegraphics[width=\linewidth]{figures/assets/prefix.pdf}
    }
    \caption{(Example 2) Prefix text used for conditional generation, extracted from the QMSum dataset~\cite{zhong2021qmsumnewbenchmarkquerybased}.}
    \label{fig:apx:prefix}
\end{figure}

\begin{figure}[t]
    \centering
    \footnotesize
    \setlength{\fboxsep}{-2pt}
    \fcolorbox{gray}{white}{%
        \includegraphics[width=\linewidth]{figures/assets/suffix.pdf}
    }
    \caption{(Example 2) Suffix text used for conditional generation, extracted from the QMSum dataset~\cite{zhong2021qmsumnewbenchmarkquerybased}.}
    \label{fig:apx:suffix}
\end{figure}

% \clearpage
\begin{figure}[t]
    \centering
    \footnotesize
    \setlength{\fboxsep}{-2pt}
    \fcolorbox{gray}{white}{%
        \includegraphics[width=\linewidth]{figures/assets/reference.pdf}
    }
    \caption{(Example 2) The ground-truth reference text extracted from the QMSum dataset~\cite{zhong2021qmsumnewbenchmarkquerybased}.}
    \label{fig:apx:reference}
\end{figure}

\begin{figure}[t]
    \centering
    \footnotesize
    \setlength{\fboxsep}{-2pt}
    \fcolorbox{gray}{white}{%
        \includegraphics[width=\linewidth]{figures/assets/prime_response.pdf}
    }
    \caption{(Example 2) Conditional sample generated using MDM-Prime-v2 (1.1B).}
    \label{fig:apx:prime_response}
\end{figure}



\begin{figure}[t]
    \centering
    \footnotesize
    \setlength{\fboxsep}{-2pt}
    \fcolorbox{gray}{white}{%
        \includegraphics[width=\linewidth]{figures/assets/ar_response.pdf}
    }
    \caption{(Example 2) Conditional sample generated using Pythia (1.4B).}
    \label{fig:apx:pythia_response}
\end{figure}



